X-ViT: High Performance Linear Vision Transformer without Softmax

Vision transformers have become one of the most important models for computer vision tasks. Although they outperform prior works, they require heavy computational resources on a scale that is quadratic to the number of tokens, $N$. This is a major drawback of the traditional self-attention (SA) algorithm. Here, we propose the X-ViT, ViT with a novel SA mechanism that has linear complexity. The main approach of this work is to eliminate nonlinearity from the original SA. We factorize the matrix multiplication of the SA mechanism without complicated linear approximation. By modifying only a few lines of code from the original SA, the proposed models outperform most transformer-based models on image classification and dense prediction tasks on most capacity regimes.

==> table/available_batch_size.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=\linewidth]{figures/available_batch_size.png}
\end{center}
\caption{\textbf{Maximum batch size on the limited memory.} Comparison of maximum available batch sizes of various models on 16GB of VRAM. We scaled batch size by 2 until the peak memory exceeds 16GB.}
\label{fig:available_batch_size}
\end{figure}

==> table/centroids_figure.tex <==
\begin{figure}[t] % t: top, b: bottom, h: here
\begin{center}
\includegraphics[width=0.7\linewidth]{figures/centroids_figure.png}
\end{center}
\caption{\textbf{Centroids generating harmonic potentials.} Each patch, represented as a particle, is interfered by parabolic potentials generated from $h$ clusters.}
\label{fig:centroids_figure}
\end{figure}
\textbf{Replace softmax to XNorm.} In XNorm, key and value of self-attention multiplied directly. It generates $h$ clusters through linear kernel method.
\begin{align}\label{eq:kv}
[K^{T}V]_{ij}=\sum^n_{k=1}K^T_{ik}V_{kj}
\end{align}

==> table/flops_acc_comparison.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=\linewidth]{figures/flops_acc_comparison.png}
\end{center}
\caption{\textbf{Top-1 accuracy vs. FLOPS.} Comparison of ImageNet1k top-1 accuracy of various models according to FLOPS. The results of models fine-tuned at higher resolutions are added. Our models show the best results at the same FLOPS compared to the other models.}
\label{fig:flops_acc_comparison}
\end{figure}


==> table/hyperparams.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}}                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}Models} \\ \cline{2-5} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Hyperparameter}} & X-ViT-T & X-ViT-S       & X-ViT-M       & X-ViT-B       \\ \hline
learning rate     & 5e-4 & 5e-4  & \multicolumn{2}{c|}{4e-4} \\ \hline
DropPath\cite{huang2016deep}         & 0.05 & 0.1   & 0.15        & 0.25        \\ \hline
RandAugment\cite{cubuk2020randaugment}      & 2, 7 & 2, 7 & 2, 9       & 3, 12       \\ \hline
\end{tabular}
\caption{\textbf{Hyperparameters for image classification.} All the other hyperparameters are same as DeiT\cite{touvron2020training}.} \label{tb:hyperparams}
\end{table*}

==> table/imagenet_ablation.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{l|c}
\hline
\rowcolor[HTML]{EFEFEF} 
Method              & Top-1 Acc. (\%) \\ \hline
Baseline(Linear Embed+XNorm)            & 81.8                       \\ \hline
XNorm $\rightarrow$ LN\cite{ba2016layer}, GN\cite{wu2018group}, IN\cite{ulyanov2016instance}          & Failed                     \\ \hline
XNorm $\rightarrow$ Learnable $p$-Norm & 81.8                       \\ \hline
XNorm $\rightarrow$ Single $L_2$-norm & Failed                       \\ \hline
Linear Embed\cite{dosovitskiy2020image} $\rightarrow$ Conv Embed         & 82.0                       \\ \hline
% +Longer Epochs      & Failed                     \\ \hline
Hyperparameter Optimization           & 82.8                       \\ \hline
\end{tabular}
\caption{\textbf{Ablation study.} The results of ablation study on ImageNet1k classification for X-ViT-M model. Note that single $L_2$-Norm means applying $L_2$-Norm to only one of query and key-value interaction.} \label{tb:imagenet_ab}
\end{table}

==> table/model_setup.tex <==
\begin{table*}[hbt!]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
\rowcolor[HTML]{EFEFEF} 
Model & Depth & \#Dim & \#Embed & \#Head & GFLOPS & Params (M) & Res. & Patch Size \\ \hline
X-ViT-T & 24 & 192 & 96 & 4 & 1.9  & 10.0 & 224 & 16 \\ \hline
X-ViT-S & 12 & 384 & 128 & 8 & 3.7  & 20.7 & 224 & 16 \\ \hline
X-ViT-M & 24 & 384 & 128 & 8 & 7.0  & 37.3 & 224 & 16 \\ \hline
X-ViT-B & 24 & 512 & 128 & 8 & 11.9 & 63.7 & 224 & 16 \\ \hline
\end{tabular}
\caption{\textbf{X-ViT models.}} \label{tb:model_setup}
\end{table*}

==> table/visualized_attention.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=\linewidth]{figures/visualized_attention.png}
\end{center}
\caption{\textbf{Visualized attentions.} Visualization of attention matrices using pseudo-inverse scheme. These matrices are extracted from class attention module of pretrained X-ViT-S. The brighter colors represent the values closer to 1. The thresholds are adjusted manually.}
\label{fig:vis_attn}
\end{figure}
